A Proof Theoretic Study of Soft Concurrent Constraint Programming

Concurrent Constraint Programming (CCP) is a simple and powerful model for concurrency where agents interact by telling and asking constraints. Since their inception, CCP-languages have been designed for having a strong connection to logic. In fact, the underlying constraint system can be built from a suitable fragment of intuitionistic (linear) logic --ILL-- and processes can be interpreted as formulas in ILL. Constraints as ILL formulas fail to represent accurately situations where "preferences" (called soft constraints) such as probabilities, uncertainty or fuzziness are present. In order to circumvent this problem, c-semirings have been proposed as algebraic structures for defining constraint systems where agents are allowed to tell and ask soft constraints. Nevertheless, in this case, the tight connection to logic and proof theory is lost. In this work, we give a proof theoretical interpretation to soft constraints: they can be defined as formulas in a suitable fragment of ILL with subexponentials (SELL) where subexponentials, ordered in a c-semiring structure, are interpreted as preferences. We hence achieve two goals: (1) obtain a CCP language where agents can tell and ask soft constraints and (2) prove that the language in (1) has a strong connection with logic. Hence we keep a declarative reading of processes as formulas while providing a logical framework for soft-CCP based systems. An interesting side effect of (1) is that one is also able to handle probabilities (and other modalities) in SELL, by restricting the use of the promotion rule for non-idempotent c-semirings.This finer way of controlling subexponentials allows for considering more interesting spaces and restrictions, and it opens the possibility of specifying more challenging computational systems.

==> logical-reading.tex <==
%!TEX root = softccp-sell.tex

In most of \ccp\ based systems, it is possible to recognize
a logical fragment (the constraint system) embedded inside an 
operational system. In~\cite{fages01ic}, it was shown
that the operational fragment could also be seen as a logical
system, establishing the connection between \ccp\ and intuitionistic linear logic. In~\cite{DBLP:conf/concur/NigamOP13}, we have enhanced this result, showing that
both: this connection is, in fact, strong (in the sense that operational steps matches {\em exactly} focused logical steps~\cite{nigam09ppdp})
and it can be extended to various \ccp\ flavors, like epistemic, 
spatial and timed.


% In Section~\ref{sec:semisub} we came back to the foundations of \ccp\ and gave, for the first time, a logical definition
% of soft constraints. In this section, we move on and present
% the logical interpretation of soft constraint processes, showing, 
% as in~\cite{DBLP:conf/concur/NigamOP13}, that 
% such an interpretation is {\em adequate}. 


Assume a soft constraint system as in Definition~\ref{def:soft-cons} and let $\Sigma$ be the subexponential signature $
 \tup{\cA \cup \{\infty,\pfamily,\dfamily\}, \preceq, \cA\cup
\infty}
$, where, for any $a,b\in\cA$, $a\preceq b$ iff $a\leq_A b$
while
$a,\pfamily,\dfamily\preceq \infty$.
Observe that $a,\infty \in U$ while $\pfamily,\dfamily\notin U$. 

Intuitively, the subexponential $\pfamily$ is used
to mark processes,  $\dfamily$ is used to mark procedures $p(\vx)$ whose
definition may be unfolded and $\infty$ marks non-logical axioms and process definitions.
Formally, \ccp\ processes, non-logical axioms and
are encoded process definitions into \sell\ as follows (\red{check that $\top_\cA$ plays the role of $\infty$})

\begin{definition}[Encoding of processes, non-logical axioms and process definitions]\label{def:se-csystem}
For any process $P$,  $\pEnc{P}{}$ is defined recursively as:
\[
\begin{array}{l@{\qquad}l}
\bullet~\pEnc{\tellp{c}}{} = \nbang{\pfamily} c &
\bullet~\pEnc{\sum\limits_{i\in I}\whenp{c_i}{P_i}}{} = \nbang{\pfamily} \bigwith_{i\in I} (c_i\limp \pEnc{P_i}{})\\
\bullet~\pEnc{\localp{\vx}{P}}{} =  \nbang{\pfamily}( \exists \vx. \pEnc{P}{}) &
\bullet~\pEnc{P_1,...,P_n}{} =\pEnc{ P_1}{}   \ot ... \ot   \pEnc{P_n}{} \\
\bullet~\pEnc{p(\vx)}{} =\nbang{\dfamily} p(\vx).
\end{array}
\]
A non-logical axiom of the form $\forall \vx (d \supset c)$ and 
a process definition of the form $p(\vx)\defsymboldelta P$
are encoded, respectively,  as:
$$
\nbang{\infty} \forall \vx. (d \limp c)
\qquad \mbox{and}\qquad
\nbang{\infty} \forall \vx.((\nbang{\dfamily}p(\vx)) \limp \pEnc{P}{})
$$
\end{definition}  
Following similar steps presented in~\cite{DBLP:conf/concur/NigamOP13} we can prove the following adequacy theorem.
We write $\enc{\Delta}$ and $\enc{\Psi}$ for the set of \sell\ formulas encoding
the non-logical axioms $\Delta$ and the process definitions $\Psi$.

\begin{theorem}
\label{thm:adeq-basic}
Let $P$ be a \ccp\  process,
$(\cC,\vdash_\Delta)$ be  an CS, $\Psi$ be a set of process definitions.
% Let $\bigtriangledown_{\ell}$ be instantiated to $\nbang{\ell}$.
Then $\Barb{P}{c}$ iff $ \enc{\Delta}, 
  \enc{\Psi}, \pEnc{P}{} \lra
c \otimes \top$.
% ~~\footnote{
% With the $\top$ unit 
% on the righthand side of the sequent  we capture the observables of a process  regardless whether the final configuration  has suspended asks processes.}. 
\end{theorem}
% The proof is on the level of derivations, where proof search from the 
% process encoding corresponds exactly to the execution the  process.
% 
% \red{EP. Not sure this is right... I think we need quantification.}


==> sell.tex <==
%!TEX root = softccp-sell.tex
We shall now 
review some basic proof theory of Girard's intuitionistic
linear logic (ILL) \cite{girard87tcs} with 
subexponentials~\cite{danos93kgc}.
ILL's connectives are the conjunctions $\tensor$ 
and $\with$; the disjunction $\plus$; the implication $\lolli$;
the (first-order) 
quantifiers 
$\forall$ and $\exists$;
the exponentials $\bang,\quest$;\footnote{Although $\quest$ is not part of ILL, we can add a linear version of it,
not allowing it to be contracted or weakened.}  
and the units $\one,\top$ and $\zero$.

Due to the exponential $\bang$, we can distinguish in linear logic
two kinds of formulas in the left context: the linear ones whose main connective is not a
$\bang$ and the unbounded ones whose main connective is a $\bang$.
It turns out that the exponentials are not canonical  
with respect to the logical equivalence relation. 
In fact, if, for any reason, we decide to define a blue  
and red conjunctions ($\wedge^b$ and $\wedge^r$ respectively) with the standard  rules:
\[
\begin{array}{l@{\qquad\qquad}l}
\infer[\wedge^b L]{\Gamma,A\wedge^b B\vdash C}
{\deduce{\Gamma,A,B\vdash C}{}}
&
\infer[\wedge^b R]{\Gamma\vdash A\wedge^b B}
{\deduce{\Gamma\vdash A}{}&
\deduce{\Gamma\vdash B}{}}\\[5pt]
\infer[\wedge^r L]{\Gamma,A\wedge^r B\vdash C}
{\deduce{\Gamma,A,B\vdash C}{}}
&
\infer[\wedge^r R]{\Gamma\vdash A\wedge^r B}
{\deduce{\Gamma\vdash A}{}&
\deduce{\Gamma\vdash B}{}}
\end{array}
\]
then it is easy to show that, for any formulas $A$ and $B$, $A\wedge^b B\equiv A\wedge^r B$.
This means that all the symbols for intuitionistic conjunction belong to the same equivalence class. Hence,
we can choose to use as the conjunction's \emph{canonical} form any particular color, 
and provability is not affected by this choice. 

However, the same behavior 
does not hold with the linear logic exponentials. In fact, suppose we have
red $\bang^r$
and blue $\bang^b$ exponentials with the standard linear logic rules:
$$\infer[\nbang{r} R]{\bang^r\Gamma\vdash\bang^r
F}{\bang^r\Gamma\vdash F}\qquad
\infer[\bang^r L]{\Gamma,\bang^r F\vdash C}{\Gamma, F\vdash C}\qquad
\infer[\bang^b R]{\bang^b\Gamma\vdash\bang^b
F}{\bang^b\Gamma\vdash F}\qquad
\infer[\bang^b L]{\Gamma,\bang^b F\vdash C}{\Gamma, F\vdash C}$$
We cannot show that $\bang^r F\equiv \bang^b F $.  
This opens the possibility of defining
classes of exponentials. 

Formally, intuitionistic linear logic with subexponentials (\sell) shares with ILL  all 
connectives and their inference rules,
except the exponentials: instead of
having a single pair of exponentials $\bang$ and $\quest$, \sell\ may
contain as many \emph{labeled} exponentials, 
 $\nbang{l},\nquest{l}$,
as needed. These are called \emph{subexponentials}~\cite{danos93kgc}. 
The \emph{subexponential signature} $\Sigma = \tup{I, \preceq, U}$ is built from  
 a set of labels $I$, $U \subseteq I$ is a set specifying which
subexponentials allow weakening and contraction
on the left side of a sequent, and $\preceq$ is the  pre-order among the elements of $I$. We assume that $U$ is closed wrt $\preceq$, \ie, if $a \in U$ and $a \preceq
b$, then $b \in U$.

The exponentials
  introduction rules are as follows. For each $a \in I$, we add
the  introduction rules corresponding to dereliction and
promotion, where we state explicitly the first-order signature $\Lscr$
of the terms of the language:
\[
\infer[\nbang{a}_L]{\Lscr;\Gamma, \nbang{a} F \lra G} {\Lscr;\Gamma, F \lra
G} \quad \textrm{ and } \quad
\infer[\nbang{a}_R]{\Lscr;\nbang{x_1} F_1, \ldots \nbang{x_n} F_n
\lra \nbang{a} G}{\Lscr;\nbang{x_1} F_1, \ldots \nbang{x_n} F_n \lra  G}
\]

\noindent
The rules for $\nquest{a}$ are dual.
Here, the rule $\nbang{a}_R$ (and $\nquest{a}_L$) have the side condition
that $a \preceq x_i$ for all $i$. That is, one can only
introduce a $\nbang{a}$ on the right (or a $\nquest{a}$ on the left) if
all other formulas in the sequent are marked with indices that are
greater or equal than $a$.  

Observe that this means that provability is preserved {\em downwards}: if a formula
$\nbang{a}P$ is provable from a set of hypothesis,
so it is $\nbang{b}P$, for  $b\preceq a$.


Furthermore, for all 
  $a \in U$, we add the  structural rules:
\[
\infer[C]{\Lscr;\Gamma, \nbang{a} F \lra G} {\Lscr;\Gamma, \nbang{a} F, \nbang{a} F
\lra G} \quad \textrm{ and } \quad
\infer[W]{\Lscr;\Gamma, \nbang{a} F \lra G} {\Lscr;\Gamma \lra G}
\]

That is, we are also free to specify which indices are \emph{unbounded} (those appearing in the set
$U$), and which indices are \emph{linear} or \emph{bounded}.
See the 
companion technical report of \cite{concur13} at the authors' web page   for a focused 
intuitionistic version of the \sellU system.

It is known  that subexponentials greatly increase
the expressiveness of the system when compared to linear logic. For instance,
subexponentials can be used to represent contexts of proof
systems~\cite{nigam11lsfa}, to mark the epistemic state of
agents~\cite{nigam12lics}, or to specify locations in sequential
computations~\cite{nigam09ppdp}. 

The key difference to standard
presentations of linear logic is that while linear logic has only seven logically
distinct prefixes of bangs and question-marks, \sell\ allows for an
unbounded number of such prefixes, \eg, $\nbang{i}$, or
$\nbang{i}\nquest{j}$. As  showed in~\cite{concur13}, by using
different prefixes,
we are able to interpret
subexponentials in more creative ways, such as temporal
units  or spatial and epistemic modalities in distributed systems. For instance, $\nbang{i}{P}$ specifies that the process $P$ is located at space $i$. Moreover, since $\nbang{i}{P} \lra P$, the information of $P$ can be propagated outside the space $i$. On the other side,   $\nbang{i}\nquest{i}{P}$  specifies that $P$ is located at $i$ but its information is  confined to the space $i$. 

The interpretation of the aforementioned modalities in \sell\ relies on the ability to quantify on subexponentials. For that, 
we introduced in \cite{concur13} the system \sellU 
containing two novel connectives: universal ($\forallLoc$) and existential ($\existsLoc$)   quantifiers over 
{\em subexponentials}. This system is described in the next section. 
%
%However, \sell\ has a serious limitation: it does not have any sort of
%quantification over subexponentials. Therefore, given the interpretation
%above for subexponentials, it is not feasible in \sell\ to specify
%properties that are valid for all locations or for all agents. Another way
%of visualizing this limitation is that any sequent in any derivation in
%$\sell$ has the same (initial) subexponential signature $\Sigma$.


